An Approach to Mispronunciation Detection and Diagnosis with Acoustic, Phonetic and Linguistic (APL) Embeddings

Many mispronunciation detection and diagnosis (MD&D) research approaches try to exploit both the acoustic and linguistic features as input. Yet the improvement of the performance is limited, partially due to the shortage of large amount annotated training data at the phoneme level. Phonetic embeddings, extracted from ASR models trained with huge amount of word level annotations, can serve as a good representation of the content of input speech, in a noise-robust and speaker-independent manner. These embeddings, when used as implicit phonetic supplementary information, can alleviate the data shortage of explicit phoneme annotations. We propose to utilize Acoustic, Phonetic and Linguistic (APL) embedding features jointly for building a more powerful MD&D system. Experimental results obtained on the L2-ARCTIC database show the proposed approach outperforms the baseline by 9.93%, 10.13% and 6.17% on the detection accuracy, diagnosis error rate and the F-measure, respectively.

==> content/5.Acknowledgements.tex <==
% \section{ACKNOWLEDGEMENTS}
% \label{sec:acknowledgements}

==> content/6.Reference.tex <==
\section{REFERENCES}
\label{sec:reference}

==> table/table_mdd.tex <==
\begin{table*}[]
\centering
\caption{Results of mispronunciation detection and diagnosis}
\label{table_mdd}
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
Models                 & FRR             & FAR              & DER              & Recall           & Precision        & F-measure        \\ \hline
CNN-RNN-CTC            & 24.45\%         & \textbf{24.81\%} & 44.14\%          & \textbf{74.19\%} & 34.70\%          & 47.28\%          \\ \hline
Baseline               & 24.19\%         & 27.60\%          & 44.07\%          & 72.40\%          & 35.29\%          & 47.45\%          \\ \hline
Baseline-fbank+AM1     & 12.12\%         & 41.83\%          & 37.67\%          & 58.17\%          & 46.66\%          & 51.78\%          \\ \hline
Baseline-fbank+AM2     & 13.55\%         & 39.43\%          & 37.64\%          & 60.57\%          & 44.89\%          & 51.57\%          \\ \hline
Baseline+AM1           & 13.57\%         & 38.01\%          & 37.89\%          & 61.99\%          & 45.43\%          & 52.44\%          \\ \hline
Baseline+AM2           & 8.88\%          & 45.51\%          & 33.94\%          & 54.49\%          & 52.79\%          & 53.62\%          \\ \hline
Baseline+AM2+Focal CTC & \textbf{8.76\%} & 45.40\%          & \textbf{32.84\%} & 54.60\%          & \textbf{53.18\%} & \textbf{53.88\%} \\ \hline
\end{tabular}
\end{table*}
